Lensing by galaxy halos in clusters of galaxies

Weak shear maps of the outer regions of clusters have been successfully used to map the distribution of mass at large radii from the cluster center. The typical smoothing lengths employed thus far preclude the systematic study of the effects of galactic-scale substructure on the measured weak lensing signal. In this paper, we present two methods to infer the possible existence and extent of dark halos around bright cluster galaxies by quantifying the `local' weak lensing induced by them. The proposed methods are: direct radial averaging of the shear field in the vicinity of bright cluster members and a maximum-likelihood method to extract fiducial parameters characterizing galaxy halos. We demonstrate using simulations that these observed local weak-shear effects on galaxy scales within the cluster can be used to statistically constrain the mean mass-to-light ratio, and fiducial parameters like the halo size, velocity dispersion and hence mass of cluster galaxies. We compare the two methods and investigate their relative drawbacks and merits in the context of feasibility of application to HST cluster data, whereby we find that the prospects are promising for detection on stacking a minimum of 20 WFPC2 deep cluster fields.

==> refs <==
%A Efstathiou G.
%A Bernstein G.
%A Tyson A.
%A Katz N.
%A Guhathakurta P.
%D 1991
%J ApJ
%V 380
%P 47
%L efsta91a

%A Smail I.
%A Hogg D.
%A Yan L.
%A Cohen J.
%D 1995
%J ApJ Lett
%V 449
%P 105
%L smail95f

%A Tremaine S.
%A Richstone D.
%A Byun Y.
%A et. al.
%D 1994
%J AJ
%V 107
%P 634
%L tremaine94

%A Byun Y.
%A Grillmair C.
%A Faber S.
%A et. al.
%D 1996
%R preprint astro-ph/9602117
%L byun96

%A Faber S.
%A Tremaine S.
%A Ajhar E.
%D 1996
%R preprint astro-ph/9610055
%L faber96

%A Madau P.
%A Ferguson H. 
%A et. al
%D 1996
%R preprint astro-ph/9607172
%L madau96

%A Zepf S.
%A Silk, J.
%D 1996
%R peprint astro-ph/9601166
%L zepf96

%A Gallego J.
%A Zamorano J.
%A Aragon-Salamanca A.
%A Rego M.
%D 1995
%R preprint astro-ph/9510061
%L gallego95

%A Pei Y.
%A Fall S. M.
%D 1995
%J ApJ
%V 454
%P 69
%L fallpei

%A Rees M.
%D 1993
%S Proceedings of the National Academy of Sciences
%C Washington D. C.
%P 4840
%L mjr93

%A Silk J.
%D 1993
%S Proceedings of the National Academy of Sciences
%C Washington D. C.
%P 4835
%L silk93

%A Wyse R.
%A Silk J.
%D 1989
%J ApJ
%V 339
%P 700
%L wysilk89

%A Efstathiou G.
%D 1995
%J MNRAS
%V 274
%P 73
%L efstalambda

%A Kochanek C.
%D 1996
%J ApJ
%V 466
%P 638
%L kochlambda

%A Dell' Antonio I.
%A Tyson A.
%D 1996
%R preprint astro-ph/9608043
%L tyson96 

%A Larson R. B. 
%D 1978
%J MNRAS
%V 184
%P 69L
%L larson

%A Loeb A.
%D 1993
%J ApjL
%V 403
%P 542
%L loeb93

%A Loeb A.
%A Rasio F.
%D 1994
%J ApjL
%V 432
%P 57
%L rasio94

%A Eisenstein D.
%A Loeb A.
%D 1995
%J ApjL
%V 448
%P 17
%L eisenstein95

%A Bartelmann M.
%D 1994 
%J A&A
%V 303
%P 643
%L bartelmann94

%A Thomas P.
%A Fabian A.
%D 1990
%J MNRAS
%V 246
%P 156
%L thomas90

%A Nulsen P.
%A Fabian A.
%D 1995
%J MNRAS
%V 277
%P 561
%L nulfab95

%A White D.
%A Forman W.
%A Jones C.
%D 1996
%R preprint
%L davwhite96

%A Heckman T. M.
%A Baum S. A.
%A Breugel van W. J. M.
%A McCarthy P.
%D 1989
%J ApJ
%V 338
%P 48
%L heckman89

%A Bower R. G.
%A Lucey J. R.
%A Ellis R. S.
%D 1992
%J MNRAS
%V 254
%P 601
%L bower92

%A Merritt D.
%D 1988
%S The Minnesota lectures on clusters of galaxies and large-scale structure
%E Dickey J.
%I ASP Conf. Series
%P 175
%L merritt88

%A Ostriker J.
%A Tremaine S.
%D 1975
%J ApJ
%V 256
%P 435
%L ostriker75a

%A Cardiel N.  
%A Gorgas J.
%A Arag\'{o}n-Salamanca A.
%D 1995
%J MNRAS
%V 277
%P 502
%L gorgas95

%A Cardiel N. 
%A Gorgas J.
%A Arag\'{o}n-Salamanca A.
%D 1996
%R Conference proceedings
%L gorgas96a

%A Cardiel N. 
%A Gorgas J.
%A Arag\'{o}n-Salamanca A.
%D 1996
%R in preparation.
%L gorgas96b

%A Blakeslee J.
%A Tonry J. L.
%D 1992
%J AJ
%V 103
%P 5 
%L blakeslee

%A Hausman M.
%A Ostriker J.
%D 1978
%J ApJL
%V 224
%P 320
%L hausman78

%A Ostriker J.
%A Hausman M.
%D 1977
%J ApJ
%V 217
%P 125
%L hausman77

%A Richstone D.
%D 1976
%J ApJ
%V 204
%P 642
%L richstone76

%A Merritt D.
%D 1984
%J ApJ
%V 276
%P 26
%L merritt86

%A Merritt D.
%D 1984
%J ApJL
%V 280
%P 5
%L merritt84

%A Evans N. W.
%A De Zeeuw T.
%D 1994
%J MNRAS
%V 271
%P 202
%L wynevans94

%A Liu F. K.
%D 1996
%J MNRAS
%V 281
%P 1197
%L liu

%A Ellis R. S.
%A Smail I. R.
%A Dressler A.
%A Couch W.
%A Oemler A.
%A Butcher H.
%A Sharples R.
%D 1996
%R preprint 
%L morphs96

%A Butcher H.
%A Oemler A.
%D 1978
%J ApJ
%V 219
%P 18
%L butcher

%A Tyson A.
%A Fischer P.
%D 1995
%J ApJ
%V 446
%P 55
%L tyson1689

%A Haynes M.
%D 1989
%S Clusters of Galaxies
%E Oegerle W. R.
%E Fitchett M. J.
%E Danly L.
%I Cambridge Univ. Press
%C Cambridge
%P 177
%L haynes89

%A Whitmore B.
%D 1989
%S Clusters of Galaxies
%E Oegerle W. R.
%E Fitchett M. J.
%E Danly L.
%I Cambridge Univ. Press
%C Cambridge
%P 139
%L whitmore89

%A Richstone D.
%D 1989
%S Clusters of Galaxies
%E Oegerle W. R.
%E Fitchett M. J.
%E Danly L.
%I Cambridge Univ. Press
%C Cambridge
%P 231
%L richstone89

%A Forman W.
%A Jones C.
%D 1989
%S Clusters of Galaxies
%E Oegerle W. R.
%E Fitchett M. J.
%E Danly L.
%I Cambridge Univ. Press
%C Cambridge
%P 257
%L forman89

%A Fitchett M. J.
%D 1989
%S Clusters of Galaxies
%E Oegerle W. R.
%E Fitchett M. J.
%E Danly L.
%I Cambridge Univ. Press
%C Cambridge
%P 111
%L fitchett89

%A Kochanek C.
%A Narayan R.
%D 1992
%J ApJ
%V 401
%P 461
%L kochanek92

%A Giovanelli R.
%A Haynes M.
%D 1988
%S Galactic and Extragalactic Astronomy
%E Verschur G. L.
%E Kellermann K. I.
%I Springer Verlag
%C New York
%P 522
%L giovanelli88

%A Haehnelt M.
%A Rees M. J.
%D 1993
%J MNRAS
%V 263
%P 168
%L haehnelt93

%A Babul A.
%A Rees M. J.
%D 1992
%J MNRAS
%V 255
%P 346
%L babul92

%A Efstathiou G.
%A Rees M. J.
%D 1988
%J MNRAS
%V 230
%P 5
%L efsta88

%A White D. A.
%A Fabian A. C.
%D 1995
%J MNRAS
%V 273
%P 72
%L dwhite

%A Arimoto N.
%A Kodama T.
%D 1996
%R preprint.
%L arimoto96

%A Ciotti L.
%D 1996
%R astro-ph/9605084
%L ciotti96

%A Carlberg R.
%D 1994
%J ApJ
%V 433
%P 468
%L carlberg1

%A White S. D. M.
%A Navarro J. F.
%A Evrard A. E.
%A Frenk C. S.
%D 1994
%J Nature
%V 366
%P 429
%L whitebary

%A Olive K.
%A Steigman G.
%D 1995
%J ApJSupp
%V 97
%P 737
%L olive

%A Chandrasekhar S.
%D 1939
%S An Introduction to the study of stellar structure
%I University of Chicago Press
%C Chicago
%P 173
%L Chandrasekhar

%A Liu F. K.
%D 1995
%R astro-ph/9512061, preprint.
%L Liu

%A Emden R.
%D 1907
%S Gaskugeln - Anwendungen der Mechan. Warmtheorie
%I Druck und Verlag Von B. G. Teubner
%C Leipzig
%P 129
%L Emden

%A Evans N. W.
%A De Zeeuw T.
%D 1994
%J MNRAS
%V 271
%P 202
%L wynevans

%A Jaffe W.
%D 1983
%J MNRAS
%V 202
%P 995
%L jaffe83

%A Smail I.
%A Ellis R. S.
%A Fitchett M. J.
%A Edge A. C.
%D 1995
%J MNRAS
%V 273
%P 277
%L smail95e

%A Glazebrook K.
%A Ellis R. S.
%A Santiago B.
%A Griffiths R.
%D 1994
%J BAAS
%V 185
%P 9505
%L glazebrook95

%A Hernquist L.
%D 1990
%J ApJ
%V 356
%P 359
%L hernquist90a

%A Natarajan P.
%A Kneib J-P.
%D 1996
%R MNRAS, in press.
%L natarajan96c

%A Abraham R. G.
%A Tanvir N. R.
%A Santiago B.
%A Ellis R. S.
%A Glazebrook K.
%A van den Bergh S.
%D 1996
%J MNRAS
%V 279
%P L47
%L abraham96

%A Lefevre O.
%A Crampton D.
%A Felenbok P.
%A Monnet G.
%D 1994
%J A&A
%V 282
%P 325
%L lefevre94

%A Bouchet F. R.
%A Hernquist L.
%D 1988
%J ApJS
%V 68
%P 521
%L bouchet88

%A Barnes J.
%A Hut P.
%D 1989
%J ApJS
%V 70
%P 389
%L barnes89

%A Hernquist L.
%A Barnes J.
%D 1990
%J ApJ
%V 349
%P 562
%L hernquist90b

%A Dyer C. C.
%A Ip P. S. S.
%D 1993
%J ApJ
%V 409
%P 60
%L dyer93

%A Peebles J.
%D 1980
%S The Large-Scale Structure of the Universe
%I Princeton University Press
%C Princeton
%L peebles80

%A Gerhard O.
%D 1993
%J MNRAS
%V 265
%P 213
%L gerhard93

%A Carlberg R.
%A Yee H. K. C.
%A Ellingson E.
%A Abraham R.
%A Gravel P.
%A Morris S.
%A Pritchet C. J.
%D 1996
%J ApJ
%V 462
%P 32
%L carlberg96

%A Merritt D.
%A Tremblay B.
%D 1994
%J AJ
%V 108
%P 514
%L merritt94	

%A Yee H. K. C.
%A Ellingson E.
%A Carlberg R.
%D 1996
%J ApJS
%V 102
%P 269
%L cnoc96

%A Jorgensen I. 
%A Franx M.
%A Kjaergaard P.
%D 1996
%J MNRAS
%V 280
%P 167
%L inger96

%A Djorgovski G.
%A Davis M.
%D 1987
%J ApJ
%V 313
%P 59
%L djorgovski87

%A Dressler A.
%A Lynden-Bell D.
%A Burstein D.
%A Davies R. L.
%A Faber S. M.
%A Terlevich R. J.
%A Wegner G.
%D 1987
%J ApJ
%V 313
%P 42
%L dressler87

%A Kassiola A.
%A Kovner I.
%A Fort B.
%D 1993
%J ApJ
%V 400
%P 41
%L kovner93

%A Broadhurst T.
%A Taylor A. N.
%A Peacock J.
%D 1995
%J ApJ
%V 438
%P 49
%L broadhurst

%A Hjorth J.
%A Kneib J-P.
%D 1996
%R in preparation
%L hjorth96 

%A Squires G.
%A Kaiser N.
%D 1995
%R astro-ph/9512094, preprint.
%L squires96

%A Natarajan P.
%A Kneib J-P.
%A Smail I.
%D 1996
%R in preparation
%L natarajan96a

%A Smail I.
%A Dressler A.
%A Kneib J-P.
%A Ellis R.
%A Couch W.
%A Sharples R.
%A Oemler A.
%D 1995
%J ApJ
%V 469
%P 508
%L smail96

%A Griffiths R.
%A Casertano S.
%A  Im M.
%A Ratnatunga K. U.
%D 1996
%R MNRAS in press.
%L griffiths96

%A Tyson J. A.
%A Valdes F.
%A Jarvis J. F.
%A Mills A. P.
%D 1984
%J ApJL
%V 281
%P 59
%L tyson84

%A Goldreich P.
%D 1984
%J ApJ
%V 281
%P 1
%L fillmore84

%A West M. J.
%A Dekel A.
%A Oemler A.
%D 1987
%J ApJ
%V 316
%P 1
%L west87

%A Navarro J.
%A Frenk C. S.
%A White S. D. M.
%D 1996
%J ApJ
%V 462
%P 563
%L navarro96

%A Navarro J.
%A Frenk C. S.
%A White S. D. M.
%D 1995
%J MNRAS
%V 275
%P 720
%L navarrox95

%A Hoffman Y.
%A Shaham J.
%D 1985
%J ApJ
%V 297
%P 16
%L hoffman85

%A Richstone D.
%A Loeb A.
%A Turner E.
%D 1992
%J ApJ
%V 393
%P 477
%L richstone92

%A Dodds S. J.
%D 1995
%R PhD thesis, University of Edinburgh
%L dodds95

%A Lynden-Bell D.
%D 1996
%R private communication
%L lynden-bell96

%A Lynden-Bell D.
%D 1967
%J MNRAS
%V 136
%P 101
%L dlb67

%A White S. D. M.
%D 1996
%S Gravitational Dynamics
%E Lahav O.
%E Terlevich E.
%E Terlevich R.
%I Cambridge Univ. Press
%C Cambridge
%P 121
%L simon96

%A Voglis N.
%D 1994
%J MNRAS
%V 267
%P 379
%L voglis

%A Binney J.
%D 1982
%J MNRAS
%V 200
%P 951
%L binney82a

%A Eddington A.
%D 1916
%J MNRAS
%V 76
%P 572
%L eddington16


%A Bartelmann M.
%A Steinmetz M.
%A Weiss A.
%D 1995
%J A&A
%V 297
%P 1
%L mathias95

%A Eke V.
%A Cole S.
%A Frenk C. S.
%A Navarro J. F.
%D 1996
%J MNRAS
%V 281
%P 703
%L eke96

%A Hoffman Y.
%A Ribak E.
%D 1991
%J ApJ
%V 380
%P 5
%L hoffman-ribak91

%A van Kampen E.
%D 1996 
%R preprint, submitted to MNRAS
%L eelco96a

%A Natarajan P.
%A Kneib J-P.
%D 1996
%R preprint, submitted to MNRAS
%L natarajan96d

%A van Kampen E.
%D 1995
%J MNRAS
%V 273
%P 295
%L eelcofirst

%A van de Weygaert R.
%A Bertschinger E.
%D 1996
%J MNRAS
%V 281
%P 84
%L rein96

%A Carlberg R.
%D 1995
%R private communication
%L carlberg95

%A van Kampen
%A Katgert P.
%D 1996
%R preprint.
%L katgert96

%A Abell 
%D 1958
%J ApJ Supp
%V 3
%P 517
%L abell58

%A Katgert P.
%A Mazure A.
%A Perea J.
%A den Hartog R.
%A et. al.
%D 1996
%J A&A
%V 310
%P 8
%L esokey95

%A Abell
%A Corwin
%A Olowin
%D 1989
%J ApJ Supp
%V 70
%P 1
%L aco90

%A Schneider P.
%A Rix H.
%D 1996
%R astro-ph/9601190, preprint.
%L schneiderrix96


%A Kriessler J.
%A Beers T.
%A Odewahn S.
%D 1995
%J BAAS
%V 186
%P 07.02
%L kriessler95

%A Griffiths R.
%A Casertano S.
%A Ratnatunga K.
%A Neuchafer L.
%D 1994
%J ApJL
%V 435
%P 19
%L griffiths94

%A West M.
%A Bothun G.
%D 1990
%J ApJ
%V 350
%P 36
%L west90

%A Bird C.
%D 1993
%J PASP
%V 105
%P 1495
%L bird93

%A Spergel D. N.
%A Hernquist L.
%D 1992
%J ApJ
%V 397
%P 75
%L spergel92

%A Hernquist L.
%A Spergel D.
%A Heyl J.
%D 1993
%J ApJ
%V 416
%P 415
%L hernquist93

%A Evrard A. 
%A Mohr J.
%A Fabricant D.
%A Geller M.
%D 1993
%J ApJL
%V 410
%P 9
%L evrard93

%A Aragon-Salamanca A.
%A Ellis R.
%D 1993
%J MNRAS
%V 262
%P 764
%L aragon93

%A Efstathiou G.
%A Bernstein G.
%A Tyson A.
%A Katz N.
%A Guhathakurta P.
%D 1991
%J ApJL
%V 380
%P 47
%L efsta91

%A Lilly S.
%A Tresse L.
%A Hammer F.
%A Crampton D.
%A Le Fevre O.
%D 1995
%J ApJL
%V 455
%P 108
%L cfrs195

%A Cole S.
%A Lacey C.
%D 1996
%J MNRAS
%V 281
%P 716
%L lacey96

%A Tormen G.
%A Bouchet F.
%A White S. D. M.
%D 1996
%R MNRAS in press.
%L tormen96

%A Carlberg R.
%A Lake G.
%A Norman C.
%D 1986
%J ApJ
%V 300
%P 1
%L carlberg86

%A van Albada T.
%D 1982
%J MNRAS
%V 201
%P 939
%L vanalbada82 

%A Frenk C.
%A White S. D. M.
%A Efstathiou G.
%A Davis M.
%D 1985
%J Nature
%V 317
%P 595
%L frenk85

%A Londrillo P.
%A Messina A.
%A Stiavelli M.
%D 1991
%J MNRAS
%V 250
%P 54
%L londrillo91

%A Merritt D.
%A Tremaine S.
%A Johnstone D.
%D 1989
%J MNRAS
%V 236
%P 829
%L merritt89


%A Stiavelli M.
%A Bertin G.
%D 1987
%J MNRAS
%V 229
%P 61
%L stiavelli85

%A Allen S.
%A Fabian A.
%A Kneib J-P.
%D 1996
%J MNRAS
%V 279
%P 615
%L allen95

%A Brainerd T.
%A Blandford R.
%A Smail I.
%D 1996
%J ApJ
%V 466
%P 623
%L brainerd95

%A Natarajan P.
%A Hjorth J.
%A Van Kampen E.
%D 1996
%R submitted
%L natarajan96b

%A Aguilar L.
%A Merritt D.
%D 1990
%J ApJ
%V 354
%P 399
%L aguilar90

%A Evrard A.
%D 1990
%J ApJ
%V 363
%P 349
%L evrard90

%A Markevitch M.
%A Mushotzky R.
%A Inoue H.
%A Yamashita K.
%A Furuzawa A.
%A Tawara Y.
%D 1996
%J ApJ
%V 456
%P 437
%L mush96

%A Tremaine S.
%A H\'{e}non M.
%A Johnstone R.
%D 1986
%J MNRAS
%V 219
%P 285
%L henon86

%A Tremaine S.
%A H\'{e}non M.
%A Lynden-Bell D.
%D 1986
%J MNRAS
%V 219
%P 285
%L tremaine86

%A Merritt D.
%A Tremaine S.
%A Johnstone R.
%D 1986
%J MNRAS
%V 236
%P 829
%L merritt86

%A Lima-Neto G.
%D 1993
%J A\&A
%L lima-neto93

%A Carlberg R.
%D 1994
%J ApJ
%V 434
%P 51
%L carlberg94

%A Fahlman G.
%A Kaiser N.
%A Squires G.
%A Woods D.
%D 1994
%J ApJ
%V 437
%P 56
%L fahlman94

%A Squires G.
%A Neumann D.
%A Kaiser N.
%A Arnaud M.
%A Babul A.
%A Bohringer H.
%A Fahlman G.
%A Woods D.
%D 1996
%R astro-ph/9603050, preprint.
%L squires2163

%A Squires G.
%A Kaiser N.
%A Fahlman G.
%A Babul A.
%A Woods D.
%D 1996
%J ApJ
%V 469
%P 73
%L squires2390
 
%A Kaiser N.
%A Squires G.
%A Broadhurst T.
%D 1995
%J ApJ
%V 449
%P 460
%L kaiser95b

%A Schneider P. 
%D 1995
%J A&A
%V 302
%P 639
%L peter95a

%A Seitz S.
%A Schneider P.
%D 1996
%J A&A
%V 305
%P 383
%L stella96

%A Seitz C.
%A Schneider P.
%D 1995
%J A&A
%V 297
%P 287
%L caro95b

%A Schneider P.
%A Seitz C.
%D 1995
%J A&A
%V 294
%P 411
%L caro95a

%A Kaiser N. 
%D 1995
%J ApJL
%V 439
%P 1
%L kaiser95a


%A Dressler A.
%D 1979
%J ApJ
%V 231
%P 659
%L dressler79

%A Ebbels T.
%A Kneib J-P.
%A Ellis R.
%D 1997
%R in prep.
%L ebbels96

%A Pello R.
%A Le Borgne J-F
%A Sanahuja B.
%A Mathez G.
%A Fort B.
%D 1992
%J A&A
%V 266
%P 6
%L pello92 

%A Bonnet H.
%A Mellier Y.
%D 1995
%J A&A
%V 303
%P 331
%L bonnet95

%A Kassiola A.
%A Kovner I.
%D 1993
%J ApJ
%V 417
%P 450
%L kassiola93

%A Yee H.
%A Ellingson E.
%A Carlberg R.
%D 1996
%R ApJS (submitted)
%L yee96

%A Miralda-Escude J.
%D 1995
%J ApJ
%V 438
%P 514
%L jme95

%A Blandford R.
%A Kochanek C.
%D 1987
%J ApJ
%V 313
%P 28
%L blandford87c

%A Bird C.
%D 1994
%J BAAS
%V 185
%P 530
%L bird94

%A Merritt D.
%A Gebhardt K.
%D 1995
%S Proc. of the XXIXth Rencontre de Moriond: Clusters of Galaxies
%E Durret F.
%I Kluwer
%C Dordrecht
%P 121
%L merritt95a

%A Moore B.
%A Katz N.
%A Lake G.
%A Dressler A.
%A Oemler A.
%D 1996
%J Nature
%V 379
%P 613
%L moore95

%A Kneib J-P.
%A Soucail G.
%D 1996
%S Astrophysical Applications of Gravitational Lensing
%E Kochanek C.
%E Hewitt J.
%I Kluwer
%C Dordrecht
%P 113
%L kneibsoucail95

%A Natarajan P.
%D 1996
%S Astrophysical Applications of Gravitational Lensing
%E Kochanek C.
%E Hewitt J.
%I Kluwer
%C Dordrecht
%P 155
%L priya96

%A Fitchett M.
%D 1988
%S The Minnesota lectures on clusters of galaxies and large-scale structure
%E Dickey J.
%I ASP Conf. Series
%P 45 
%L fitchett88

%A Aragon-Salamanca A.
%A Ellis R.
%A Couch W.
%A Carter D.
%D 1993
%J MNRAS
%V 262
%P 764
%L alfonso93

%A Binney J.
%D 1977
%J MNRAS
%V 181
%P 735
%L binney77

%A Binney J.
%A Mamon G.
%D 1982
%J MNRAS
%V 200
%P 361
%L binneymamon82

%A Nulsen P.
%D 1986
%J MNRAS
%V 221
%P 377
%L nulsen86

%A Barnes J.
%D 1996
%S Formation of the Galactic Halo - Inside and Out
%E Morrison H. L.
%E Sarajedini A.
%I ASP Conf. Series
%C Dordrecht
%P 415
%L barnes96

%A Tremaine S.
%D 1987
%S Structure and Dynamics of Elliptical Galaxies
%E De Zeeuw T.
%I IAU Symp. 127
%C Dordrecht
%P 367
%L tremaine87

%A White S. D. M.
%D 1987
%S Structure and Dynamics of Elliptical Galaxies
%E De Zeeuw T.
%I IAU Symposium 127
%C Dordrecht
%P 339
%L white87

%A Bicknell G. 
%A Carter D.
%A Killeen N.
%A Bruce T.
%D 1989
%J ApJ
%V 336
%P 639
%L bicknell89

%A Fabian A.
%A Johnstone R.
%A Daines S.
%D 1994
%J MNRAS
%V 271
%P 737
%L fabian94a

%A Navarro J.
%A White S. D. M.
%D 1994
%J MNRAS
%V 267
%P 401
%L navarro94a

%A Crone M.
%A Evrard A.
%A Richstone D.
%D 1994
%J ApJ
%V 434
%P 402
%L crone94

%A Barnes J.
%A Hernquist L.
%D 1992
%J ARA&A
%P 705
%L barnes93

%A Frenk C.
%A Evrard A.
%A White S. D. M.
%A Summers F.
%D 1995
%R astro-ph/9504020, preprint
%L frenk95

%A Kormendy J.
%D 1989
%J ApJL
%V 342
%P L63
%L kormendy89 

%A White S. D. M.
%A Navarro J.
%A Evrard A.
%A Frenk C.
%D 1993
%J Nature
%V 366
%P 429
%L white93

%A Cen R.
%D 1994
%J ApJ
%V 437
%P 12
%L cen94

%A Klypin A.
%A Holtzmann J.
%A Primack J.
%A Reg\"{o}s E.
%D 1993
%J ApJ
%V 416
%P 1
%L klypin

%A Cen R.
%A Gnedin N.
%A Ostriker J.
%D 1993
%J ApJ
%V 415
%P 423
%L cen93

%A Navarro J.
%A Frenk C.
%A White S. D. M.
%D 1994
%J MNRAS
%V 267
%P 1
%L navarro94b

%A Hjorth J.
%A Madsen J.
%D 1991
%J MNRAS
%V 253
%P 703
%L hjorth91

%A Hjorth J.
%A Madsen J.
%D 1995
%J ApJ
%V 445
%P 55
%L hjorth95

%A Bertin E.
%D 1995
%R Sextractor Manual
%L bertin95a

%A Bertin E.
%A Arnouts S.
%D 1995
%R preprint
%L bertin95b

%A Reisenegger A.
%A Miralda-Escude J.
%A Waxman E.
%D 1996
%J ApJ
%V 457
%P 11
%L reisenegger95

%A Birkinshaw M.
%A Hughes J.
%D 1994
%J ApJ
%V 420
%P 33
%L birkinshaw94

%A Fisher D.
%A Illingworth G.
%A Franx M.
%D 1995
%J ApJ
%V 438
%P 539
%L fisher95

%A Fried J.
%A Illingworth G.
%D 1994
%J AJ
%V 107
%P 992
%L fried94

%A Fort B.
%A Mellier Y.
%D 1994
%J AARA
%V 5
%P 239
%L fort94

%A Jones M.
%A Saunders R.
%A Alexander P.
%A Birkinshaw M.
%A Dilon N.
%A Grainge K.
%A Hancock S.
%A Lasenby A.
%A Lefevre D.
%A Pooley G.
%D 1993
%J Nature
%V 365
%P 320
%L jones93

%A Holtzmann J.
%A Burrows C.
%A Casertano S.
%A Hester J.
%A Trauger J.
%A Watson A.
%A Worthey G.
%D 1995
%R preprint 
%L holtzmann95

%A Kassiola A.
%A Kovner I.
%D 1993
%J ApJ
%V 417
%P 450
%l kassiola93

%A Kassiola A.
%A Kovner I.
%D 1992
%J ApJ
%V 400
%P 41
%L kassiola92

%A King C.
%A Ellis R.
%D 1995
%J ApJ
%V 288
%P 456
%L king95
 
%A Kneib J-P.
%A Mellier Y.
%A Fort B.
%A Mathez G.
%D 1993
%J AAP
%V 273
%P 367
%L kneib93c
 
%A Kneib J-P.
%A Mellier Y.
%A Fort B.
%A Soucail G.
%A Longaretti P.
%D 1994
%J AAP
%V 286
%P 701
%L kneib93d

%A Kochanek C.
%D 1990
%J MNRAS
%V 247
%P 135
%L kochanek90

%A Kochanek C.
%D 1994
%J ApJ
%V 436
%P 56
%L kochanek94

%A Le Borgne J.
%A Pell\'o R.
%A Sanahuja B.
%D 1992
%J A&AS
%V 95
%P 87
%L leborgne92a

%A Mellier Y.
%A Fort B.
%A Kneib J-P.
%D 1993
%J ApJ
%V 407
%P 33
%L mellier93

%A Smail I.
%A Couch W.
%A Sharples R.
%D 1995
%J ApJ
%V 440
%P 501
%L smail95a

%A Smail I.
%A Dressler A.
%A Kneib J-P.
%A Ellis R.
%A Couch W.
%A Sharples R.
%A Oemler A.
%D 1995
%R ApJ, submitted
%L smail95b

%A Smail I.
%A Hogg D.
%A Blandford R.
%A Cohen J.
%A Edge A.
%A Djorgovski S.
%D 1995
%R MNRAS, in press
%L smail95c

%A Smail I.
%A Hogg D.
%A Lin Yan
%A Cohen J.
%D 1995
%J ApJL
%V 449
%P 105
%L smail95d

%A Zabludoff A.
%A Geller M.
%D 1994
%J AJ
%V 107
%P 1929
%L zablu94a

%A Bernstein G.
%A Guhathakurta P.
%A Raychaudhary S.
%A Giovanelli R.
%A Haynes M.
%A Herter T.
%A Vogt N.
%D 1994
%J AJ
%V 107
%P 1962
%L bernstein94

%A Odewahn S. C.
%A Aldering G.
%D 1995
%J AJ
%V 110
%P 2009
%L odewahn95

%A Zabludoff A.
%A Franx M.
%A Geller M.
%D 1993
%J ApJ
%V 419
%P 47
%L zablu93c

%A Zabludoff A.
%A Franx M.
%D 1993
%J AJ
%V 106
%P 1314
%L zablu93a

%A Lynden-Bell D.
%D 1967
%J MNRAS
%V 136
%P 101
%L lyndenbell67a

%A White S. D. M.
%D 1976
%J MNRAS
%V 177
%P 717
%L white76a

%A Hoyle F.
%D 1953
%J ApJ
%V 118
%P 513
%L hoyle53

%A Zabludoff A.
%A Geller M.
%A Huchra J.
%A Vogeley M.
%D 1993
%J AJ
%V 106
%P 1273
%L zablu93b

%A Zabludoff A.
%A Geller M.
%A Huchra J.
%D 1990
%J ApJ
%V 74
%P 1
%L zablu90

%A Gunn J.
%A Gott R.
%D 1972
%J ApJ
%V 176
%P 1
%L gunn72

%A Bahcall J.
%A Sarazin C.
%D 1977
%J ApJL
%V 213
%P L99
%L bahcall77

%A Fabian A.
%A Hu E.
%A Cowie L.
%A Grindlay J.
%D 1981
%J ApJ
%V 248
%P 47
%L fabian81

%A Fabian A.
%A Nulsen P.
%D 1977
%J MNRAS
%V 180
%P 479
%L nulsen77

%A Fabian A.
%A Nulsen P.
%D 1978
%J MNRAS
%V 186
%P 783
%L nulsen78

%A Kneib J-P.
%A Mellier Y.
%A Pell\'{o} R.
%A Miralda-Escud\'{e} J.
%A Le Borgne J.
%A B\"{o}hringer H.
%A Picat J.
%D 1995
%J A&A
%V 303
%P 27
%L kneib95a

%A Briel U.
%A Henry J.
%D 1995
%J Nature
%V 372
%P 439
%L briel95

%A Nulsen P.
%A B\"{o}hringer H.
%D 1995
%J MNRAS
%V 274
%P 1093
%L nulsen95

%A Bower R.
%A B\"{o}hringer H.
%A Briel H.
%A Ellis R.
%A Castander F.
%A Couch W.
%D 1994
%J MNRAS
%V 268
%P 345
%L bower94

%A Efsthathiou G.
%A Frenk C.
%A Davis M.
%A White S. D. M.
%D 1985
%J ApJS
%V 57
%P 241
%L efdw85

%A Kneib J-P.
%A Ellis R.
%A Smail I.
%A Couch W.
%A Sharples R.
%D 1996
%J ApJ 
%V 471
%P 643
%L kneib96

%A Colless M.
%A Dunn A.
%D 1996
%J ApJ
%V 458
%P 435
%L colless95

%A Waxman E.
%A Miralda-Escud\'{e} J.
%D 1995
%J ApJ
%V 451
%P 451
%L waxman95

%A Kaiser N.
%A Squires G.
%D 1993
%J ApJ
%V 404
%P 441
%L kaiser93
 
%A  Millington S.
%A  Peach J.
%D 1986
%J MNRAS
%V 221
%P 15
%L millington&peach92

%A Sharples R. 
%A Ellis R.
%A Gray P.
%D 1988
%J MNRAS
%V 231
%P 479
%L sharples88

%A Le Borgne J.
%A Pell\'{o} R.
%A Sanahuja B.
%D 1992
%J ApJ Supp
%V 95
%P 87
%L leborgne92b

%A Kent S. 
%A Sargent W.
%D 1983
%J AJ
%V 88
%P 697
%L kent83

%A Kent S. 
%A Gunn J.
%D 1982
%J AJ
%V 87
%P 945
%L kent82

%A Merritt D. 
%D 1987
%J ApJ
%V 313
%P 121
%L merritt87

%A The L.
%A White S. D. M.
%D 1988
%J AJ
%V 95
%P 15
%L the88

%A The L.
%A White S. D. M.
%D 1986
%J AJ
%V 92
%P 1248
%L the86

%A Ostriker J.
%A Tremaine S.
%D 1975
%J ApJL
%V 202
%P 113
%L ostriker75

%A Peebles J.
%D 1971
%J AA
%V 11
%P 377
%L peebles71a

%A Peebles J.
%D 1969
%J ApJ
%V 155
%P 393
%L peebles69a

%A van den Bergh S.
%D 1976
%J ApJ
%V 206
%P 883
%L vandenberg76

%A Fabian A.
%A Nulsen P.
%A Canizares C.
%D 1982
%J MNRAS
%V 201
%P 933
%L fabian82

%A Dressler A.
%D 1980
%J ApJ
%V 236
%P 351
%L dressler80a

%A Fabian A.
%A Schwarz J.
%A Forman W.
%D 1980
%J MNRAS
%V 192
%P 135
%L fabian80b

%A Fabian A.
%D 1994
%J ARAA
%V 32
%P 277
%L fabian94b

%A White D. A.
%A Fabian A.
%D 1994
%J MNRAS
%V 273
%P 72
%L whited94

%A Doroshkevich A.
%D 1973
%J ApJL
%V 14
%P 11
%L doroshkevich73

%A Squires G.
%A Kaiser N.
%A Fahlman G.
%A Woods D.
%A Babul A.
%D 1996
%J ApJ
%V 461
%P 572
%L squires95

%A Binney J.
%A Tremaine S.
%D 1987
%S Galactic Dynamics
%I Princeton Univ. Press
%C Princeton
%L b&t87

%A Rees M.
%D 1993
%S Perspectives in Astrophysical Cosmology
%I Cambridge Univ. Press
%C Cambridge
%L mjrbook

%A Chandrasekhar S.
%D 1939
%S An Introduction to the study of stellar structure
%I University of Chicago Press
%C Chicago
%L chandra39

%A Press W.
%A Teukolsky S.
%A Vettering W.
%A Flannery B.
%D 1992
%S Numerical Recipes
%I Cambridge University Press
%C Cambridge
%L press92

%A Kneib J-P.
%D 1993
%S PhD Thesis
%C Universit\'{e} de Toulouse III
%L kneib93b

%A Sarazin C.
%D 1988
%S X-ray emissions from clusters of galaxies
%I Cambridge Univ. Press
%C Cambridge
%L sarazin88

%A Peebles J.
%D 1993
%S Principles of Physical Cosmology
%I Princeton Univ. Press
%C Princeton
%L peebles93

%A Chandrasekhar S.
%D 1939
%S An Introduction to the theory of stellar structure
%I University of Chicago Press
%C Chicago
%L chandra39

%A Blandford R.
%A Narayan R.
%D 1986
%J ApJ
%V 310
%P 568
%L blandford87a












































